A JWST Study of the Remarkable Oort Cloud Comet C/2017 K2 (PanSTARRS)

Comets, during their journeys into the inner solar system, deliver volatile gases, organics, and particulates into their comae that provide crucial information for assessing the physico-chemical conditions in the outer disk from which they formed. Here we present observational and modeling results of a JWST NIRSpec and MIRI MRS integral-field-unit (IFU) spatial-spectral study of the inner coma of the Oort Cloud comet C/2017 K2 (PanSTARRS) at a heliocentric distance of 2.35 au. We find the comet is hyperactive (water ice active fraction greater than or equal to 86%), with a nucleus radius of $<$4.2 km, exhibiting strong emission from H$_{2}$O, $^{12}$CO, $^{13}$CO, and CO$_{2}$ as well as CN, H$_2$CO, CH$_3$OH, CH$_4$, C$_2$H$_6$, HCN, NH$_2$, and OH prompt emission. The water ortho-to-para ratio is greater than or equal to 2.75. The modeled dust composition (relative mass fraction of the sub-micron grains) in the coma is dominated by amorphous carbon ($\simeq 25$%), amorphous Mg:Fe olivine ($\simeq 19$%), amorphous Mg:Fe pyroxene ($\simeq 16$%), and Mg-rich crystalline olivine ($\simeq 39$%) and the crystalline mass fraction of the sub-micron grains in the coma is, $f_{cryst} \simeq 0.384 \pm 0.065$. Analysis of residuals in 3 to 8 $\mu$m region of the spectral energy distribution strongly suggests the presence of polycyclic aromatic hydrocarbon (PAHs) species in the coma.

==> figset-10.tex <==
\figsetstart
\figsetnum{10}
\figsettitle{Model fits to H$_{2}$O, CO$_{2}$, $^{13}$CO$_{2}$, CO, CH$_{4}$, 
CH$_{3}$OH, HCN, OCS, and C$_{2}$H$_{6}$ emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS). }

\figsetgrpstart
\figsetgrpnum{10.1}
\figsetgrptitle{Model fits to H$_{2}$O 2.9~\micron}
\figsetplot{fig10-a-h20-2.9um.pdf}
\figsetgrpnote{Model fits to H$_{2}$O 2.9~\micron{} emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.2}
\figsetgrptitle{Model fits to H$_{2}$O 5.9~\micron}
\figsetplot{fig10-b-h20-5.0um.pdf}
\figsetgrpnote{Model fits to H$_{2}$O 5.9~\micron{}  emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.3}
\figsetgrptitle{Model fits to CO$_{2}$}
\figsetplot{fig10-c-CO2.pdf}
\figsetgrpnote{Model fits to CO$_{2}$ emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{10.4}
\figsetgrptitle{Model fits to $^{13}$CO$_{2}$}
\figsetplot{fig10-d-13CO2.pdf}
\figsetgrpnote{Model fits to $^{13}$CO$_{2}$ emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.5}
\figsetgrptitle{Model fits to CO}
\figsetplot{fig10-e-CO.pdf}
\figsetgrpnote{Model fits to CO emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.6}
\figsetgrptitle{Model fits to CH$_{4}$}
\figsetplot{fig10-f-CH4.pdf}
\figsetgrpnote{Model fits to CH$_{4}$ emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.7}
\figsetgrptitle{Model fits to CH$_{3}$OH}
\figsetplot{fig10-g-CH3OH.pdf}
\figsetgrpnote{Model fits to  CH$_{3}$OH emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.8}
\figsetgrptitle{Model fits to HCN}
\figsetplot{fig10-h-HCN.pdf}
\figsetgrpnote{Model fits to HCN emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.9}
\figsetgrptitle{Model fits to OCS}
\figsetplot{fig10-i-OCS.pdf}
\figsetgrpnote{Model fits to OCS emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{10.10}
\figsetgrptitle{Model fits to C$_{2}$H$_{6}$}
\figsetplot{fig10-j-C2H6.pdf}
\figsetgrpnote{Model fits to C$_{2}$H$_{6}$ emission derived from the NIRSpec spectra of C/2017 K2 (PanSTARRS).
(Top panel pair) The extracted on-nucleus spectrum.  (Bottom panel pair) The extracted off-nucleus spectrum (-1:-1) position 
(see Figure~\ref{fig:mrs-beamtile-positions} that describes the spatial location of the beams). 
Measurements and model fits are shown in black and red, respectively, while the residual is shown in green.
Derived apparent production rate (for H$_{2}$O) or abundance relative to H$_{2}$O (for all other species) at 
each position is indicated. The derived or assumed (in parentheses) rotational temperature are listed in the inset.}
\figsetgrpend

\figsetend


==> figset-15.tex <==
\figsetstart
\figsetnum{15}
\figsettitle{The  \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture within the coma of comet C/2017 K2 (PanSTARRS). }

\figsetgrpstart
\figsetgrpnum{15.1}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:0}
\figsetplot{fig15-1_tile_00_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the photocenter (position 0:0) of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.2}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:-1}
\figsetplot{fig15-2_tile_0m1_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position 0:-1 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.3}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:+1}
\figsetplot{fig15-3_tile_0p1_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position 0:+1 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.4}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition -1:0}
\figsetplot{fig15-4_tile_m10_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position -1:0 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.5}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition -1:-1}
\figsetplot{fig15-5_tile_m1m1_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position -1:-1 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.6}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition +1:0}
\figsetplot{fig15-6_tile_p10_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position +1:0 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{15.7}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition +1:+1}
\figsetplot{fig15-7_tile_p1p1_c17k2ps_ao50favor_jwst_mrs_v1140_1227pmap_c17k2ps_DEH_Model+Residuals_chmerged_scaled_box1d.pdf}
\figsetgrpnote{(Top panel). The \textbf{`AO50'} thermal model fitted to the JWST MRS IR SED  in a 1\farcs0 diameter 
aperture centered on the tile position +1:+1 of comet C/2017 K2 (PanSTARRS). (Bottom Panel) The model 
residual (observed data - best fit thermal model) is in the bottom panel. The spectral region containing the $\nu_{2}$ water 
emission bands (purple, bottom panel) were not included in the model fit, and the grey vertical regions illustrated the point-point 
uncertainties (discussed in Section~\ref{sec:sec-dust-model-3cases}).}
\figsetgrpend

\figsetend


==> figset-18.tex <==
\figsetstart
\figsetnum{18}
\figsettitle{The relative mass fraction of comet C/2017 K2 (PanSTARRS) in 1\farcs0 diameter beam within the coma.}

\figsetgrpstart
\figsetgrpnum{18.1}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:0}
\figsetplot{fig18-1_pie_massfrac_tile_00_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position 0:0.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.2}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:-1}
\figsetplot{fig18-2_pie_massfrac_tile_0m1_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position 0:-1.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.3}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition 0:+1}
\figsetplot{fig18-3_pie_massfrac_tile_0p1_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position 0:+1.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.4}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition -1:0}
\figsetplot{fig18-4_pie_massfrac_tile_m10_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position -1:0.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.5}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition -1:-1}
\figsetplot{fig18-5_pie_massfrac_tile_m1m1_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position -1:-1.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.6}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition +1:0}
\figsetplot{fig18-6_pie_massfrac_tile_p10_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position +1:0.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{18.7}
\figsetgrptitle{C2017/K2 (PanSTARRS) TilePosition +1:+1}
\figsetplot{fig18-7_pie_massfrac_tile_p1p1_ao50favor_v1140_1227pmap_jwst_mrs_c2017k2ps_DEH_Model.pdf}
\figsetgrpnote{The relative mass fraction for the submicron- to micron- size portion of the particle differential size distribution in 
the inner coma of comet C/2017 K2 (PanSTARRS) derived from the ‘AO50’ Case C models. Tile position +1:+1.}
\figsetgrpend

\figsetend

